On the Duality of Task and Actor Programming Models

Programming models for distributed and heterogeneous machines are rapidly growing in popularity to meet the demands of modern workloads. Task and actor models are common choices that offer different trade-offs between development productivity and achieved performance. Task-based models offer better productivity and composition of software, whereas actor-based models routinely deliver better peak performance due to lower overheads. While task-based and actor-based models appear to be different superficially, we demonstrate these programming models are duals of each other. Importantly, we show that this duality extends beyond functionality to performance, and elucidate techniques that let task-based systems deliver performance competitive with actor-based systems without compromising productivity. We apply these techniques to both Realm, an explicitly parallel task-based runtime, as well as Legion, an implicitly parallel task-based runtime. We show these techniques reduce Realm's overheads by between 1.7-5.3x, coming within a factor of two of the overheads imposed by heavily optimized actor-based systems like Charm++ and MPI. We further show that our techniques enable between 1.3-5.0x improved strong scaling of unmodified Legion applications.

==> comptime.tex <==
\begin{center}
\begin{tabular}{ c c c }
   & Stencil & MiniAero & Pennant & CG \\ 
 1 & 96796ns & 138346ns & 190436ns & 325768ns \\  
 2 & 551064ns & 633452ns & 519369ns & avg(562788,587663)ns \\
 4 & 2270897ns & 1972696ns & 1525724ns & avg(534082,854492,861662,603686)ns \\
 8 & 8006942ns & 6903378ns & 5962388ns & avg(650683,891004,915155,932098,908865,881927,880984,615574) ns \\
 16 & avg(37697144, 34615463)ns & avg(13377301,13551259)ns & avg(11802710,11003906)ns & avg(641619,944534,860600,938702,902263,903030,892496,855777,986374,969259,920716,925273,912368,896470,918518,637979)ns \\
 32 & avg(34357440, 62432828, 67484447, 38068604)ns & avg(22041515,34744821,35025038,21727827)ns & avg(11576282,17807232,18175620,11915967)ns & avg(644847,972942,935451,947993,939594,912775,1012860,931889,915680,938841,975276,906196,890617,991374,928953,973076,890892,903454,909419,888172,992036,921651,911308,970066,921597,943845,929653,955496,858358,935677,924080,646459)ns \\
\end{tabular}
\end{center}

% Notes:
% * Stencil has interesting graph optimization sizes -- the "middle" nodes have longer compilation times as the middle nodes do twice as much synchronization as the interior nodes.

==> old.tex <==
\begin{figure}
\begin{lstlisting}
map<int, pair<Actor*, Processor>> all_actors;
class Actor {
  void register_with_runtime(int actor_id, Processor target) {
    all_actors[id] = {this, target};
  }
};
struct ActorTaskArgs {
  int msg_id;
  Actor* actor;
};
void actor_task(TaskRuntime* rt, void* args, int arglen) {
  int msg = (ActorTaskArgs*)(args)->msg_id;
  ActorRuntime art(rt);
  (ActorTaskArgs*)(args)->actor->handle_message(
    msg, &art, (char*)(args) + sizeof(ActorTaskArgs));
}
const int ACTOR_TASK_ID = 0;
class ActorRuntime {
  ActorRuntime(TaskRuntime* _rt) : rt(_rt) {}
  void initialize() {
    // Perform an all-gather to exchange local actor information.
    rt->register_task(ACTOR_TASK_ARGS, actor_task);
  }
  void send_message(int actor_id, int msg_id, void* args, int arglen) {
    pair<Actor*, Processor> target = all_actors[actor_id];
    void* new_args = malloc(arglen + sizeof(ActorTaskArgs));
    (ActorTaskArgs*)(new_args)->msg_id = msg_id;
    (ActorTaskArgs*)(new_args)->actor = target.first;
    memcpy((char*)(new_args) + sizeof(ActorTaskArgs), args, arglen);
    rt->launch_task(target.second, ACTOR_TASK_ID, new_args, arglen + sizeof(ActorTaskArgs), {});
    free(new_args);
  }
  TaskRuntime* rt;
};

\end{lstlisting}
\caption{Actor Runtime With Task Runtime}
\end{figure}

\begin{figure}
\begin{lstlisting}
const int META_ACTOR_ID = 0;
\end{lstlisting}
\caption{Task Runtime With Actor Runtime}
\end{figure}


\section{Background}

In this section, we provide the necessary background on task-based
and actor-based programming models.
%
For each model, we present a simple calculus to describe the core
features of the programming model.
%
We then use the definitions of these models in \TODO{\Cref{TODO}} to 
discuss the duality between these two different models of distributed computation.

\subsection{Task-Based Programming Models}

The core concept in task-based programming models is a \emph{task},
which is a stateless, user-defined function.
%
Tasks may launch other tasks, and are issued onto a target processor
to run asynchronously from the launching task.
%
Task-based applications express their desired computation as a graph
of tasks that operate over shared data structures.

\Cref{fig:task-based-calculus} contains the definition of a standard
lambda calculus with mutable state extended with several constructs
for task-based programming.
%
\TODO{Probably need to restrict ourselves to a first-order calculus
to avoid issues with higher order functions flying around the network.}
%
During evaluation, an application may launch a task onto a target processor,
allocate data into a target memory, or issue a copy between two allocations
(which may possibly be in different memories).
%
Each described operation may be executed asynchronously, and as such
returns an \emph{event} (or a \emph{future}) which represents the completion of that operation.
%
Each asynchronous operation may be preconditioned on a set of events that
must all complete before the asynchronous operation begins.
%
\TODO{remove event waiting as this makes the translation annoying.}
%
Finally, an application may wait on the completion of a set of events.
%
The operational semantics for this calculus can be defined as a transition
relation between machine states, and are straightforward: every processor
may either be idling or executing a task; tasks are queued until their precondition
events are completed, and then move into a ready queue for the target processor.

The calculus presented in \Cref{fig:task-based-calculus} models an explicitly-parallel
task-based system, such as Realm~\cite{realm}, where the programmer is responsible
for specifying dependencies between parallel computations.
%
Implicitly-parallel task-based systems, such as Legion~\cite{legion} or StarPU~\cite{starpu},
instead leverage a higher-level program representation where tasks describe what data
they will access, and then perform a dependence analysis to infer the necessary 
dependencies between launched tasks.
%
These higher-level systems can represent the task graph after the dependence analysis
using a form of the presented calculus.

\TODO{rohany: Could simplify the task calculus by having just one pending queue, rather
than one per processor?}

\begin{figure}
\centering
\small
% \footnotesize
% \scriptsize
\[
\textbf{Syntax}
\]
\quad
\[
\begin{array}{rlcl} 
    \textsf{Processor} & p & & \\
    \textsf{Memory} & m & & \\
    \textsf{Types} & \tau & \bnfdef & \ldots \bnfalt \textsf{event} \\
    \textsf{Expressions} & e & \bnfdef & \ldots \bnfalt \\
                         &   &         & e : \textsf{event} = \textsf{task}(p, f, \overline{e})~\textsf{in}~e \bnfalt \\
                         % TODO (rohany): I think it's also probably simpler to not include
                         %  copies and just talk about it in the extensions section.
                         &   &         & e : \textsf{event} = \textsf{copy}(e, e, \overline{e})~\textsf{in}~e \bnfalt \\
                         % TODO (rohany): I don't know if I want to show the semantics for deferred allocation,
                         %  as it slightly complicates things for no reason (i.e. queues per memory etc).
                         &   &         & a : \textsf{ref}(\tau),~e : \textsf{event} = \textsf{alloc}(m, \overline{e})~\textsf{in}~e \bnfalt \\
                         % I think that it's simpler for us to not include wait.
                         % &   &         & \textsf{wait}(\overline{e})~\textsf{in}~e \\
    % \texttt{Partition} & P & \bnfdef & \textsf{blocks}(T, s) \bnfalt \textsf{mma}(T) \\
\end{array}
\]
\quad\quad
\[
\textbf{Operational Structures}
\]
\quad
\[
\begin{array}{rlcl} 
\textsf{Evaluation Context} & C & \bnfdef & \square \bnfalt (e, \textsf{event}) \\
% TODO (rohany): Maybe drop copies here?
\textsf{Pending Tasks} & Q^p & \bnfdef & (\textsf{task}, \textsf{event})~\textsf{list} \\
\textsf{Ready Tasks} & Q^r & \bnfdef & (\textsf{task}, \textsf{event})~\textsf{list} \\
\textsf{Completed Events} & E & \bnfdef & \textsf{event}~\textsf{set}\\
\textsf{Machine State} & \mathbb{M} & \bnfdef & ((p, C, Q^p, Q^r)~\textsf{set}, m~\textsf{set}, E) \\
\end{array}
\]
\quad\quad
\textbf{Operational Semantics}
\quad
\begin{mathpar}
\inferrule{
M, e \mapsto e', M'
}{
(\{(p, (e, ev), Q^p, Q^r), \ldots\}, M, E) \mapsto (\{(p, (e', ev), Q^p, Q^r), \ldots\}, M', E)
}{}\\
\inferrule{
M, e \mapsto v, M'
}{
(\{(p, (e, ev), Q^p, Q^r), \ldots\}, M, E) \mapsto (\{(p, \square, Q^p, Q^r), \ldots\}, M', E \cup \{ev\})
}{}\\
\inferrule{
}{
(\{(p_1, e_1 : \textsf{event} = \textsf{task}(p_2, f, \overline{e})~\textsf{in}~e_2, Q^p_1, Q^r_1), \ldots\}, M, E) \mapsto  \\
(\{(p_1, e_2, Q^p_1, Q^r_1), (p_2, C, Q^p_2 + (\textsf{task}(p_2, f, \overline{e}), e_1), Q^r_2), \ldots\}, M, E)
}\\
\inferrule{
\forall ev \in \overline{ev}, ev \in E
}{
(\{(p, C, (\textsf{task}(p, f, \overline{ev}), ev_f) :: Q^p, Q^r) \ldots\}, M, E) \mapsto  \\
(\{(p, C, Q^p, Q^r + (\textsf{task}(p, f, \overline{ev}), ev_f)) \ldots\}, M, E)
}\\
\inferrule{
}{
(\{(p, \square, Q^p, (\textsf{task}(p, f, \overline{ev}), ev_f) :: Q^r) \ldots\}, M, E) \mapsto  \\
(\{(p, (f(), ev_f), Q^p, Q^r) \ldots\}, M, E)
}\\

\end{mathpar}
\caption{Simple task-based language.}
\label{fig:task-based-calculus}
\end{figure}

\subsection{Actor-Based Programming Models}
\begin{figure}
\centering
\small
% \footnotesize
% \scriptsize
\textbf{Syntax}
\[
\begin{array}{rlcl} 
    \textsf{Processor} & p & & \\
    \textsf{Message ID} & id & & \\
    % I think the right thing here is a record type, but its a bit ugly
    % to write out.
    \textsf{Actor} & a & \bnfdef & id \times (\tau \rightarrow \textsf{unit})~\textsf{set} \\
    \textsf{Types} & \tau & \bnfdef & \ldots \bnfalt a \\
    \textsf{Expressions} & e & \bnfdef & \ldots \bnfalt () = \textsf{send}(a, id, e)~\textsf{in}~e \\
\end{array}
\]
\quad\quad
\textbf{Operational Structures}
\quad
\[
\begin{array}{rlcl} 
\textsf{Mutable Store} & S && \\
\textsf{Incoming Message Set} & M & \bnfdef & (\textsf{id}, e)~\textsf{list} \\
\textsf{Evaluation Context} & C & \bnfdef & \square \bnfalt e \\
\textsf{Actor Context} & AC & \bnfdef & (a, p, S, M, C) \\
\textsf{Machine State} & \mathbb{M} & \bnfdef & AC~\textsf{set} \\
\end{array}
\]
\quad\quad
\textbf{Operational Semantics}
\quad
\begin{mathpar}
\inferrule{
S, e \mapsto e', S'
}{
\{(a, p, S, M, e), \ldots \} \mapsto \{(a, p, S', M, e'), \ldots \}
}\\
\inferrule{
S, e \mapsto (), S'
}{
\{(a, p, S, M, e), \ldots \} \mapsto \{(a, p, S', M, \square), \ldots \}
}\\
\inferrule{
}{
\{(a_1, p_1, S_1, M_1, () = \textsf{send}(a_2, id, e_1)~\textsf{in}~e_2), (a_2, p_2, S_2, M_2, C_2), \ldots \} \mapsto \\
\{(a_1, p_1, S_1, M_1, e_2), (a_2, p_2, S_2, M_2 + (id, e_1), C_2), \ldots \}
}\\
\inferrule{
  (id, f) \in a
}{
\{(a, p, S, (id, e) :: M, \square), \ldots \} \mapsto \{(a, p, S, M, f(e)), \ldots \}
}\\
\end{mathpar}
% \quad
% \[
% \mathbb{M}, \Gamma \mapsto \mathbb{M}', \Gamma'
% \]
\caption{Simple actor-based language.}
\label{fig:actor-based-calculus}
\end{figure}

The actor programming model is characterized by a series
of stateful objects called \emph{actors} that maintain
arbitrary local state and communicate through asynchronous
message passing.
%
In modern actor-based programming systems, actors are associated
with particular machine resources, and actor-based applications
express computations through individual actors performing
local computations and notifying other actors to start follow-up work.

Actor-based programming models are well-studied and have been 
extensively formalized in prior work~\cite{agha-actors, actors-grief}.
%
For simplicity and the focus of this work, we consider
in \Cref{fig:actor-based-calculus} a simplified
actor model that is embedded within a standard host language
(such as Charm++~\cite{charm++} or Ray~\cite{ray})
and elide the object-oriented aspects of common actor formalizations.
%
As with the presentation of task-based languages, we consider
a standard lambda calculus with mutable state extended with an
\emph{actor} type, which is a record mapping message identifiers
to handler functions.
%
The main computational primitive added to the calculus is a message send
operation, which asynchronously invokes the desired function on the target
actor.
%
For simplicity,  we assume that there is some universal and static set of actors
present at program startup, and each actor is assigned to a processor.
%
In practice, most actor systems allow for the dynamic creation of new actors~\cite{charm, charm++, ray}.
%
The operational semantics for this actor calculus are similar to the
task-based calculus, where processors in the machine execute the handler
functions for actors as incoming messages arrive.
%
However, each actor only makes modifications to a local state; all communication
between actors occurs through message passing.

The actor calculus presented in \Cref{fig:actor-based-calculus} \ldots 

\begin{figure}
% TODO (rohany): Copies?
\begin{lstlisting}
class TaskRuntime {
  class Event, Allocation, Processor, Memory;
  Event launch_task(
    Processor p, int task_id, void* args, int arglen, vector<Event> pre);
  Event alloc(
    Memory m, size_t size, Allocation& result, vector<Event> pre);
  void register_task(
    int task_id, void (*task) (TaskRuntime*, void*, int));
};
// Example task:
void gpu_task(TaskRuntime*, void* args, int arglen) {
  // Stateless task body.
}
\end{lstlisting}
\caption{Task-based Runtime System}
\end{figure}

\begin{figure}
\begin{lstlisting}
class ActorRuntime {
  class Processor;
  void send_message(int actor_id, int msg_id, void* args, int arglen);
};
class Actor {
  void register_with_runtime(int actor_id, Processor target);
  virtual void handle_message(int msg_id, ActorRuntime* rt, void* args);
  // Actors may maintain arbitrary, but private state.
};
\end{lstlisting}
\caption{Actor-based Runtime System}
\end{figure}


\subsection{Task Graph Representation}

%
\begin{figure}
% TODO (rohany): This is ugly ... 
\begin{lstlisting}
struct Operation {
  enum OpKind {
    TASK,
    COPY,
    EXT_PRECOND,
    EXT_POSCOND
  } kind;
  UniqueID id;
  union {
    struct Task {
      int id;
      void* args;
    } task;
    struct Copy {
      Allocation src;
      Allocation dst;
    } copy;
    struct ExtPrecond {
      int index;
    } ext_pre;
    struct ExtPostcond {
      int index;
    } ext_post;
  } data;
};

struct SubgraphDefn {
  vector<Operation> nodes;
  vector<pair<UniqueID, UniqueID>> edges;
};

int create_subgraph(SubgraphDefn& defn);
Event launch_subgraph(
  int id, const vector<Event>& preconds, vector<Event>& postconds);
\end{lstlisting}
\caption{Simplified Static Task Graph API}
\label{fig:simple-task-graph-api}
\end{figure}

We present a simplified API for a static task graph representation in
\Cref{fig:simple-task-graph-api}.
%
The representation itself is relatively standard, and mimics static task
graph representations found in CUDA Graphs~\cite{cuda-graphs} or Ray's compiled graphs~\cite{ray-dag}.
%
A static task graph contains a vector of nodes, which may be operations like tasks or copies,
and a vector of pairs that represent dependence edges between operations.
%
The task graph representation also contains a notion of \emph{external} pre-conditions
and post-conditions.
%
External pre-conditions are dependence edges that come from operations
outside the static task graph, and external post-conditions are dependence
edges that are triggered from within the task graph and consumable by
operations outside of the graph.
%
The external pre-conditions and post-conditions act as a boundary between
static components of the subgraph amenable to optimization
with actors and dynamic components that rely on the flexibility of the
full task-based runtime system.
